NN-VVC: Versatile Video Coding boosted by self-supervisedly learned image coding for machines

The recent progress in artificial intelligence has led to an ever-increasing usage of images and videos by machine analysis algorithms, mainly neural networks. Nonetheless, compression, storage and transmission of media have traditionally been designed considering human beings as the viewers of the content. Recent research on image and video coding for machine analysis has progressed mainly in two almost orthogonal directions. The first is represented by end-to-end (E2E) learned codecs which, while offering high performance on image coding, are not yet on par with state-of-the-art conventional video codecs and lack interoperability. The second direction considers using the Versatile Video Coding (VVC) standard or any other conventional video codec (CVC) together with pre- and post-processing operations targeting machine analysis. While the CVC-based methods benefit from interoperability and broad hardware and software support, the machine task performance is often lower than the desired level, particularly in low bitrates. This paper proposes a hybrid codec for machines called NN-VVC, which combines the advantages of an E2E-learned image codec and a CVC to achieve high performance in both image and video coding for machines. Our experiments show that the proposed system achieved up to -43.20% and -26.8% Bj{\o}ntegaard Delta rate reduction over VVC for image and video data, respectively, when evaluated on multiple different datasets and machine vision tasks. To the best of our knowledge, this is the first research paper showing a hybrid video codec that outperforms VVC on multiple datasets and multiple machine vision tasks.

==> figures/fig_adapters.tex <==
\begin{figure*}[ht]
  \begin{minipage}[b]{\linewidth}
    \centering
      \centerline{\includegraphics[width=\linewidth]{figures/graphs/IHA_IMA.pdf}}
       
  \end{minipage}
  \centerline{High level structure of the adapters}

  \begin{minipage}[b]{\linewidth}
    \centering
      \centerline{\includegraphics[width=\linewidth]{figures/graphs/IHA_IMA_resblocks.pdf}}
       
  \end{minipage}
  \centerline{Resblocks component}
  
    \caption{Adapter components}
    \label{fig:adapters}
  
\end{figure*}

==> figures/fig_output_samples.tex <==
%!!! We need some visualizations of the output samples added here nicely, those can be found from "figures/visualizations"

\begin{figure*}[ht]
    \centering
    \begin{minipage}[b]{0.32\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{figures/visualizations/uncompressed_RacehorseD_intra.png}}
    %\subcaption{example}
    \centerline{Uncompressed frame 0}      
    \end{minipage}
    \begin{minipage}[b]{0.32\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{figures/visualizations/QP47_RacehorseD_output_intra-frame_plain-VVC.png}}
    \centerline{Anchor frame 0 (intra)}      
    \end{minipage}
  \begin{minipage}[b]{0.32\linewidth}
    \centering
      \centerline{\includegraphics[width=\linewidth]{figures/visualizations/QP47_RacehorseD_LIC_output_intra-frame.png}}
      \centerline{NN-VVC frame 0 (intra)}
  \end{minipage}
  
\begin{minipage}[b]{0.32\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{figures/visualizations/uncompressed_RacehorseD_inter.png}}
  \centerline{Uncompressed frame 0}     
  \end{minipage}
  \begin{minipage}[b]{0.32\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{figures/visualizations/QP47_RacehorseD_output_inter-frame1_plain-VVC.png}}
  \centerline{Anchor frame 1 (inter)}      
  \end{minipage}
  \begin{minipage}[b]{0.32\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{figures/visualizations/QP47_RacehorseD_output_inter-frame1_IHA1_IMA1.png}}
  \centerline{NN-VVC frame 1 (inter)}       
  \end{minipage}

\caption[]{Input and output samples from SFU Racehorses (Class D) at QP47} [!!!nees a bit more details in this caption to makes it easier to grasp the idea without reading the text somewhere else
!!!]
\label{fig:output_samples_sfu}
\end{figure*}

